Network Comparison: Embeddings and Interiors

This paper presents methods to compare networks where relationships between pairs of nodes in a given network are defined. We define such network distance by searching for the optimal method to embed one network into another network, prove that such distance is a valid metric in the space of networks modulo permutation isomorphisms, and examine its relationship with other network metrics. The network distance defined can be approximated via multi-dimensional scaling, however, the lack of structure in networks results in poor approximations. To alleviate such problem, we consider methods to define the interiors of networks. We show that comparing interiors induced from a pair of networks yields the same result as the actual network distance between the original networks. Practical implications are explored by showing the ability to discriminate networks generated by different models.

==> Versions/V3_package/sec_0_abstract.tex <==
%!TEX root = journal_network_embedding.tex

\begin{abstract}
This paper presents methods to compare networks where relationships between pairs of nodes in a given network are defined. We define such network distance by searching for the optimal method to embed one network into another network, prove that such distance is a valid metric in the space of networks modulo permutation isomorphisms, and examine its relationship with other network metrics. The network distance defined can be approximated via multi-dimensional scaling, however, the lack of structure in networks results in poor approximations. To alleviate such problem, we consider methods to define the interiors of networks. We show that comparing interiors induced from a pair of networks yields the same result as the actual network distance between the original networks. Practical implications are explored by showing the ability to discriminate networks generated by different models. 
\end{abstract}

% keywords
\begin{IEEEkeywords} Network theory, networked data, network comparison, metric spaces, pattern recognition
\end{IEEEkeywords}

==> Versions/V3_package/sec_1_introduction.tex <==
%!TEX root = journal_network_embedding.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   I   N   T   R   O   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Introduction}\label{sec_intro}

The field of network science is predicated on the empirical observation that network structure carries important information about phenomena of interest. Network structures haven been observed to be fundamental in social organizations \cite{Wasserman1994} and differences in the structure of brain networks have been shown to have clinical value in neurology and psychology \cite{??}. The fundamental value of network structure has led to an extensive literature on network identification that is mostly concerned with the identification of network features that serve as valuable discriminators in different contexts. Examples of these features and application domains are clustering coefficients \cite{Wang2012} and motifs \cite {Choobdar2012} in social networks; neighborhood topology \cite{Singh2008}, betweenness \cite{Peng2010}, and wavelets \cite{Yong2010} in protein interaction networks; as well as  graphlet degree distributions or signatures in different contexts \cite{Przulj2007, Milenkovic2008, Shervashidze2009}. \red{References \cite{Przulj2007, Milenkovic2008} are on protein networks. Please remove and replace with a couple of examples of features that are used to compare brain networks or some other type of network. Adapt the sentence accordingly.} However valuable, it is material to recognize that it is possible for very different networks to be indistinguishable from the perspective of specific features, or, conversely, to have similar networks that differ substantially on the values of some features. One way to sidestep this limitation it to define and evaluate proper network distances. This is the objective of this paper.

Without getting into the details of how a valid distance might be defined, it is apparent that their computation is bound to be  combinatorial. Indeed, since permutations of unlabeled nodes result in identical networks distances must rely on comparison between a combinatorial number of node correspondences -- evaluating distances is relatively simpler if nodes are labeled \cite{Onnela2007, Kossinets2006, Khmelev2001}. An important observation in this regard is that the space of finite metric spaces is a subset of the space of networks composed of those whose edges satisfy the triangle inequality. This observation is pertinent because there is a rich literature on the comparison of metric spaces that we can adopt as a basis for generalizations that apply to the comparison of networks. Of particular interest here are the Gromov-Hausdorff distance, which measures the size of the smallest modification that allows the spaces to be mapped onto each other \cite{Memoli2008}, and the partial embedding distance, which measures the size of the smallest modification that allows a space to be embedded in the other \cite{bronstein2006, bronstein2006a, bronstein2006b, memoli2004}. The computation of either of these distances is intractable. However, Gromov-Hausdorff distances can be tractably approximated using homological features \cite{Memoli2008} and embedding distances can be approximated using multi-dimensional scaling (MDS) \cite{bronstein2006}. \red{Is it possible to separate references here so that we have different papers for definitions and methods for approximation? I am sure we can do that for the GH distance. I suppose there may be a mathematical paper or book where the embedding distance is defined.} 

In prior work we have defined generalizations of the Gromov-Hausdorff distance \cite{Carlsson2014, Huang2015} and utilized homological features for computationally tractable approximate evalutions \cite{Huang2016}. Our starting point here is the partial embedding distance for metric spaces \cite{bronstein2006, bronstein2006a, bronstein2006b, memoli2004}. Our goal is to generalize embedding distances to arbitrary networks and utilize MDS techniques for their approximate computation. 

\subsection{Organization and contributions}

Networks, metrics, embedding metrics, and the Gromov-Hausdorff distance for networks are defined in Section \ref{sec_preliminaries}. The issue of defining an embedding distance for networks is addressed in Section \ref{sec_embedding_distance}. The idea of an embedding distance $d(a,b)$ is to analyze how much we have to modify network $a$ to make it a subset of network $b$. This is an asymmetric relationship. In particular, having $d(a,b) = 0$ means that network $a$ can be embedded in network $b$ but the opposite need not be true. The first contribution of this paper is to:

\begin{itemize}
\item[(i)] Define network \textit{embeddings} and a corresponding notion of partial embedding distances. Partial embedding distances define an embedding metric $d$ such that $d(a,b) = 0$ if and only if $a$ can be embedded in $b$.
\end{itemize}

We attempt to use the MDS techniques in \cite{bronstein2006} to approximate the computation of embedding distances but observe that the methodology yields poor results -- see Figure \ref{fig_mds_original} for an illustration of why this is not unexpected. To improve these results we observe that when edge dissimilarities satisfy a triangle inequality, an Euclidean interior is implicitly defined. In the case of arbitrary networks this is not true and motivates the definition of the interior of a network that we undertake in Section \ref{sec_space_induced}. The second contribution of this paper is to:

\begin{itemize}
\item[(ii)] Provide a definition of the \textit{interior} of a network. The interior of a set of nodes is the set of points that can be written as convex combinations of the nodes. The dissimilarity between points in the interior is the difference between the convex combinations of the respective dissimilarities between the respective points. 
\end{itemize}

Having the ability to extend networks into their interiors, we extend different networks and compute partial embedding distances between their extensions. In principle, distances between two networks and their respective extensions need not be related. In Section \ref{sec_interior_distance} we show that a restriction in the embedding of the extended networks renders them identical. Our third and most important contribution is to:

\begin{itemize}
\item[(iii)] Define embeddings for extended networks such that points in one of the original networks -- prior to extension -- can only be embedded into original points of the other network. We show that the embedding distance that results from this restriction is the same embedding distance between the original networks.
\end{itemize}

We point out that a network extension is a dense set that includes all the convex combinations of sets of points. To make interior extensions practical we consider samplings of the interior in Section \ref{sec_partial_embedding_induced}. It is not difficult to show in light of Contribution (iii) that the embedding distance between a a pair of networks extended to samples of their interiors is also identical to the embedding distance between the original pair of networks -- if the restriction in the mapping of original nodes is retained.

We exploit contributions (ii) and (iii) to approximate the computation of embedding distances using the MDS techniques in  \cite{bronstein2006} but applied to networks extended to their interiors. The definition of a interior markedly improves the quality of MDS distance approximations. We illustrate this fact in Section \ref{sec_application} with an artificial illustrative example and also demonstrate the ability to discriminate networks with different generative models. Although interiors are defined for sets with an arbitrary number of points, we don't use sets with more than three points in our numerical results. We further observe that it is sufficient to sample a small number of points in the interior of the network. In the numerical analyses only three points are sampled in the interior of each set of three points.



==> Versions/V3_package/sec_2_preliminaries.tex <==
%!TEX root = journal_network_embedding.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Preliminaries}\label{sec_preliminaries}

A network is defined as a pair $N_X=(X, r_X)$, where $X$ is a finite set of nodes and $r_X : X^2 = X \times X \rightarrow \reals_+$ is a function encoding dissimilarity between pairs. For $x,x'\in X$, values of this function are denoted as $r_X(x, x')$. We assume that $r_X(x, x') = 0$ if and only if $x = x'$ and we further restrict attention to symmetric networks where $r_X(x, x') = r_X(x', x)$ for all pairs of nodes $x, x' \in X$. The set of all such networks is denoted as $\ccalN$.

When defining a distance between networks we need to take into consideration that permutations of nodes amount to relabelling nodes and should be considered as same entities. We therefore say that two networks $N_X = (X, r_X)$ and $N_Y = (Y, r_Y)$ are isomorphic whenever there exists a bijection $\phi: X \rightarrow Y$ such that for all points $x, x' \in X$,
%
\begin{align} \label{eqn_network_order_2_isomorphism}
   r_X(x, x') = r_Y(\phi(x), \phi(x')).
\end{align}
%
Such a map is called an isometry. Since the map $\phi$ is bijective, (\ref{eqn_network_order_2_isomorphism}) can only be satisfied when $X$ is a permutation of $Y$. When networks are isomorphic we write $N_X \cong N_Y$. The space of networks where isomorphic networks $N_X \cong N_Y$ are represented by the same element is termed the set of networks modulo isomorphism and denoted by $\ccalN \mod \cong$. The space $\ccalN \mod \cong$ can be endowed with a valid metric \cite{Carlsson2014, Huang2015}. The definition of this distance requires introducing the prerequisite notion of correspondence \cite[Def. 7.3.17]{Burago01}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_correspondence}
A correspondence between two sets $X$ and $Y$ is a subset $C \subseteq X \times Y$ such that $\forall~x \in X$, there exists $y \in Y$ such that $(x,y) \in C$ and $\forall~ y \in Y$ there exists $x \in X$ such that $(x,y) \in C$. The set of all correspondences between $X$ and $Y$ is denoted as $\ccalC(X,Y)$.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A correspondence in the sense of Definition \ref{dfn_correspondence} is a map between node sets $X$ and $Y$ so that every element of each set has at least one correspondent in the other set. Correspondences include permutations as particular cases but also allow mapping of a single point in $X$ to multiple correspondents in $Y$ or, vice versa. Most importantly, this allows definition of correspondences between networks with different numbers of elements. We can now define the distance between two networks by selecting the correspondence that makes them most similar as stated next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_conventional_network_distance}
Given two networks $N_X = (X, r_X)$ and $N_Y = (Y, r_Y)$ and a correspondence $C$ between the node spaces $X$ and $Y$ define the network difference with respect to $C$ as 
%
\begin{align}\label{eqn_conventional_network_distance_prelim}
    \Gamma_{X,Y} (C) \!
         := \! \max_{(x, y), (x', y') \in C} 
            \Big| r_X(x, x') - r_Y (y, y') \Big|.
\end{align}
%
The network distance between $N_X$ and $N_Y$ is then defined as
%
\begin{align}\label{eqn_conventional_network_distance}
   d_\C(N_X, N_Y) := \min_{C \in \ccalC(X,Y)} 
    \Big\{ \Gamma_{X,Y} (C) \Big\}.
\end{align} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
For a given correspondence $C \in \ccalC(X,Y)$ the network difference $\Gamma_{X,Y}(C)$ selects the maximum distance difference $|r_X(x_1, x_2) - r_Y (y_1, y_2)|$ among all pairs of correspondents -- we compare $r_X(x_1, x_2)$ with $r_Y (y_1, y_2)$ when the points $x_1$ and $y_1$, as well as the points $x_2$ and $y_2$, are correspondents. The distance in \eqref{eqn_conventional_network_distance} is defined by selecting the correspondence that minimizes these maximal differences. The distance in Definition \ref{dfn_conventional_network_distance} is a proper metric in the space of networks modulo isomorphism. It is nonnegative, symmetric, satisfies the triangle inequality, and is null if and only if the networks are isomorphic \cite{Carlsson2014, Huang2015}. For future reference, the notion of metric is formally stated next. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_metric}
Given a space $\ccalS$ and an isomorphism $\cong$, a function $d : \ccalS \times \ccalS \rightarrow \reals$ is a metric in $\ccalS \mod \cong$ if for any $a, b, c \in \ccalS$ the function $d$ satisfies:
\begin{mylist}
\item [(i) {\bf Nonnegativity.}] $d(a,b) \ge 0$.
\item [(ii) {\bf Symmetry.}] $d(a,b) = d(b,a)$.
\item [(iii) {\bf Identity.}] $d(a,b) = 0$ if and only if $a \cong b$.
\item [(iv) {\bf Triangle inequality.}] $d(a,b) \le d(a,c) + d(c,b)$.
\end{mylist}\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A metric $d$ in $\ccalS\mod\cong$ gives a proper notion of distance. Since zero distances imply elements being isomorphic, the distance between elements reflects how far they are from being isomorphic. The distance in Definition \ref{dfn_conventional_network_distance} is a metric in space $\ccalN \mod \cong$. Observe that since correspondences may be between networks with different number of elements, Definition \ref{dfn_conventional_network_distance} defines a distance $d_\C(N_X, N_Y)$ when the node cardinalities $|X|$ and $|Y|$ are different. In the particular case when the functions $r_X$ satisfy the triangle inequality, the set of networks $\ccalN$ reduces to the set of metric spaces $\ccalM$. In this case the metric in Definition \ref{dfn_conventional_network_distance} reduces to the Gromov-Hausdorff (GH) distance between metric spaces. The distances $d_\C(N_X, N_Y)$ in \eqref{eqn_conventional_network_distance} are valid metrics even if the triangle inequalities are violated by $r_X$ or $r_Y$ \cite{Carlsson2014, Huang2015}.

A related notion is that of an isometric embedding. We say that a map $\phi: X \rightarrow Y$ is an isometric embedding from $N_X = (X, r_X)$ to $N_Y = (Y, r_Y)$ if \eqref{eqn_network_order_2_isomorphism} holds for all points $x, x' \in X$. Since $r_X(x, x') = r_Y(\phi(x), \phi(x'))$ for any $x, x' \in X$, $r_X(x, x') > 0$ for $x \neq x'$ and $r_Y(y, y) = 0$, the map $\phi$ is injective. This implies that the condition can only be satisfied when $N_X = (X, r_X)$ is a sub-network of $N_Y = (Y, r_Y)$. Such a map is called an isometric embedding. When $N_X$ can be isometrically embedded into $N_Y$, we write $N_X \sqsubseteq N_Y$. Related to the notion of isometric embedding is the notion of an embedding metric that we state next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_embedding_metric}
Given a space $\ccalS$ and an isometric embedding $\sqsubseteq$, a function $d : \ccalS \times \ccalS \rightarrow \reals$ is an embedding metric in $\ccalS$ if for any $a, b, c \in \ccalS$ the function $d$ satisfies:
\begin{mylist}
\item [(i)   {\bf Nonnegativity.}] $d(a,b) \ge 0$.
\item [(ii)  {\bf Embedding identity.}] $d(a,b) = 0$ if and only if $a \sqsubseteq b$.
\item [(iii) {\bf Triangle inequality.}] $d(a,b) \le d(a,c) + d(c,b)$.
\end{mylist}\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
It is apparent that metrics are embedding metrics because bijections are injective, and that in general embedding metrics are not metrics because they are asymmetric. In this paper, we consider defining an embedding distance between networks and its relationship with the Gromov-Hausdorff distance (Section \ref{sec_embedding_distance}). We then consider the problem of augmenting the networks by adding points to fill their ``interior.'' The interior is defined in such a way that embedding metrics between the original networks and embedding metrics between these augmented spaces coincide (Section \ref{sec_space_induced}).




==> Versions/V3_package/sec_3_embedding.tex <==
%!TEX root = journal_network_embedding.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Embeddings}\label{sec_embedding_distance}

As is the case with correspondences, mappings also allow definition of associations between networks with different numbers of elements. We use this to define the distance from one network to another network by selecting the mapping that makes them most similar as we formally define next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_partial_embedding}
Given two networks $N_X = (X, r_X)$, $N_Y = (Y, r_Y)$, and a map $\phi: X \rightarrow Y$ from node space $X$ to the node space $Y$, define the network difference with respect to $\phi$ as 
%
\begin{align}\label{eqn_dfn_partial_embedding_prelim}
    \Delta_{X,Y} (\phi)
         :=  \max_{x, x' \in X} 
            \Big| r_X(x, x') - r_Y (\phi(x),\phi(x')) \Big|.
\end{align}
%
The partial embedding distance from $N_X$ to $N_Y$ is defined as
%
\begin{align}\label{eqn_dfn_partial_embedding}
   d_\PE(N_X, N_Y) := \min_{\phi: X \rightarrow Y} 
    \Big\{ \Delta_{X,Y} (\phi) \Big\}.
\end{align} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Both, Definition \ref{dfn_conventional_network_distance} and Definition \ref{dfn_partial_embedding} consider a mapping between the node space $X$ and the node space $Y$, compare dissimilarities, and set the network distance to the comparison that yields the smallest value in terms of maximum differences. The distinction between them is that in \eqref{eqn_conventional_network_distance_prelim} we consider correspondence, which requires each point in any node spaces ($X$ or $Y$) to have a correspondent in the other node space, whereas in \eqref{eqn_dfn_partial_embedding_prelim} we examine mappings, which only require all points in node space $X$ to have one correspondent in the node set $Y$. Moreover, in \eqref{eqn_conventional_network_distance_prelim}, a node $x\in X$ may have multiple correspondents, however, in \eqref{eqn_dfn_partial_embedding_prelim}, a node $x\in X$ can only have exactly one correspondent. Except for this distinction, Definition \ref{dfn_conventional_network_distance} and Definition \ref{dfn_partial_embedding} are analogous since $\Delta_{X,Y}(\phi)$ selects the difference $|r_X(x_1, x_2) - r_Y(y_1, y_2)|$ among all pairs. The distance $d_\PE(N_X, N_Y)$ is defined by selecting the mapping that minimizes these maximal differences. We show in the following proposition that the function $d_\PE : \ccalN \times \ccalN \rightarrow \reals_+$ is, indeed, an embedding metric in the space of networks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition}\label{prop_partial_embedding_metric}
The function $d_\PE : \ccalN \times \ccalN \rightarrow \reals_+$ defined in \eqref{eqn_dfn_partial_embedding} is an embedding metric in the space $\ccalN$. \end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} See Appendix \ref{apx_proof_1} for proofs in Section \ref{sec_embedding_distance}. \end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The embedding distance $d_\PE(N_X, N_Y)$ from one network $N_X$ to another network $N_Y$ is not a metric due to its asymmetry. We can construct a symmetric version from $d_\PE(N_X, N_Y)$ by taking the maximum from the embedding distance $d_\PE(N_X, N_Y)$ and $d_\PE(N_Y, N_X)$. This would give us a valid metric distance in $\ccalN \mod \cong$. A formal definition and theorem statement are shown next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_embedding}
Given two networks $N_X = (X, r_X)$, $N_Y = (Y, r_Y)$, define the embedding distance between the pair as
%
\begin{align}\label{eqn_dfn_embedding}
   d_\EE(N_X, N_Y) := \max\left\{ d_\PE(N_X, N_Y), d_\PE(N_Y, N_X)\right\}.
\end{align} 
%
where partial embedding distances $d_\PE(N_X, N_Y)$ and $d_\PE(N_X, N_Y)$ are defined in Definition \ref{dfn_partial_embedding}.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem}\label{thm_embedding_distance_metric}
The function $d_\EE : \ccalN \times \ccalN \rightarrow \reals_+$ defined in \eqref{eqn_dfn_embedding} is a metric in the space $\ccalN \mod \cong$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[t]
\centerline{\input{figures/embedding_example.tex}\vspace{-1mm} 
}
\begin{minipage}[h]{0.032\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_original.eps}
\end{minipage}
\begin{minipage}[h]{0.054\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_original.eps}
\end{minipage}
\begin{minipage}[h]{0.054\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_original.eps}
\end{minipage}
\caption{An example where different networks result in identical multi-dimensional scaling results. We emphasize that the number of dimension used in multi-dimensional scaling would not distinguish networks since the triangle inequality property for relationship between nodes in the networks are violated. Such a caveat would be solved by inducing semimetrics in the space defined by the given networks, as we develop throughout Section \ref{sec_space_induced}. \vspace{-4mm}
}
\label{fig_mds_original}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Since embedding distances between two networks generate a well-defined metric, they provide a means to compare networks of arbitrary sizes. In comparing the embedding distance in \eqref{eqn_dfn_embedding} with the network distance in \eqref{eqn_conventional_network_distance} we see that both find the bottleneck that prevents the networks to be matched to each other. It is not there surprising to learn that they satisfy the relationship that we state in the following lemma. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   L   E   M   M   A   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{lemma_GH}\red{Why is this a lemma?}
The network distance $d_\C(N_X, N_Y)$ defined in \eqref{eqn_conventional_network_distance} can also be written as
%
\begin{align}\label{eqn_lemma_GH}
    d_\C(N_X, N_Y) \! = \!\!\! \min_{\substack{\phi:X \rightarrow Y\\ \psi:Y \rightarrow X}}\!\!\! 
        \max\left\{\! \Delta_{X, Y}(\phi),\! \Delta_{Y, X}(\psi),\! \delta_{X, Y}(\phi,\! \psi)\!\right\}\!,
\end{align}
%
where the network differences $\Delta_{X, Y}(\phi)$ and $\Delta_{Y, X}(\psi)$ with respect to mappings $\phi$ and $\psi$ are defined in \eqref{eqn_dfn_partial_embedding_prelim} and $\delta_{X, Y}(\phi, \psi)$ measures how far the mappings $\phi$ and $\psi$ are from being the inverse of each other, and is defined as
\begin{align}\label{eqn_lemma_GH_difference_mapping}
    \delta_{X, Y}(\phi, \psi) = \max_{x \in X, y \in Y} \left| r_X(x, \psi(y)) - r_Y(\phi(x), y) \right|.
\end{align}
%
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A direct consequence of Lemma \ref{lemma_GH} is that the embedding distance  \eqref{eqn_dfn_embedding} is a lower bound of the network distance \eqref{eqn_conventional_network_distance}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   C   O   R   O   L   L   A   R   Y   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{corollary}\label{coro_lower_bound}
Function $d_\EE$ is a lower bound with $d_\C$ in \eqref{eqn_conventional_network_distance}, i.e. 
%
\begin{align}\label{eqn_equivalence}
    d_\EE(N_X, N_Y) \leq d_\C(N_X, N_Y),
\end{align}
%
for any networks $N_X$ and $N_Y$. 
\end{corollary}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centerline{\input{figures/points_inside_network.tex}\vspace{-4mm} 
}
\caption{An example of induced space with points defined in the original network. We would like to induce a space $(S_X, s_X)$ such that $S_X$ includes infinite number of points formed by the convex of the original points $a$, $b$, and $c$, and $s_X$ is a semimetric for any pair of points in $S_X$. We want to induce the semimetric from the original network such that $s_X(a, b) = r_X(a, b)$, $s_X(a, c) = r_X(a, c)$, and $s_X(b, c) = r_X(b, c)$. Middle points, e.g. $e$, can be considered as the entity represents $50\%$ of $a$ and $50\%$ of $b$. An important observation is that any points in the space, e.g. $m$, can be written as a convex combination representing the proportion of their contents from original nodes -- $(m_a, m_b, m_c)$ with $m_a + m_b + m_c = 1$.\vspace{-4mm}
}
\label{fig_inside_example}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The relationships in Lemma \ref{lemma_GH} and Corollary \ref{coro_lower_bound} are extensions of similar analyses that hold for the Gromov-Hausdorff distance between metrics spaces, \cite{kalton1997, linial1995}. As in the case of metric spaces, these results imply that the embedding distance $d_\EE(N_X, N_Y)$ can be used to lower bound the network distance $d_\C(N_X, N_Y)$ [cf. \eqref{eqn_equivalence}]. This value is in addition to the ability of the partial embedding distance $d_\PE(N_X, N_Y)$ of Definition \ref{dfn_partial_embedding} to measure how far the network $X$ is to being a subnetwork of network $Y$.

In the comparison of surfaces and shapes, the partial embedding distance $d_\PE(N_X, N_Y)$  has the attractive property of being approximable using multidimensional scaling techniques \cite{bronstein2006, bronstein2006b}. Our empirical analysis shows that the use of analogous techniques to estimate $d_\PE(N_X, N_Y)$ for arbitrary networks shields poor results and that this is related to how far the dissimilarities in $N_X$ and $N_Y$ are from satisfying the triangle inequality -- see the example in Figure \ref{fig_mds_original} and the numerical analysis in Section \ref{sec_application}. To improve the accuracy of multidimensional scaling estimates we propose to define the interior of a network by defining a space where dissimilarities between any pair of points represented by a convex combination of nodes in the given networks are defined (Section \ref{sec_space_induced}). We will further demonstrate that the proposed definition of the interior of a network is such that the partial embedding distances between networks with interiors are the same as the partial embedding distances between the corresponding original networks (theorems \ref{thm_induced_space_distance_same} and \ref{thm_sampled_induced_space}). Empirical demonstrations will show that the comparison of networks with interiors using multidimensional scaling techniques yields better results that are comparable to those obtained when comparing shapes and surfaces (Section \ref{sec_application}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{remark}\label{remark_lower_bound}\normalfont
Another observation from Lemma \ref{lemma_GH} is that the two network distances are equivalent with $d_\EE \equiv d_\C$ if and only if the third term $\delta_{X, Y}(\phi, \psi)$ on the right hand side of \eqref{eqn_lemma_GH} is no greater than the maximum of the distances $\Delta_{X, Y}(\phi)$ and $\Delta_{Y, X}(\psi)$ measured by each of them, for the pair of mappings achieving the minimum in \eqref{eqn_lemma_GH}. In other words, the two networks can be mapped by a pair of mappings $\phi$ and $\psi$ such that the pair of maps are not that different from being inverse of each other.
\end{remark}




==> Versions/V3_package/sec_4_interiors.tex <==
%!TEX root = journal_network_embedding.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Interiors}\label{sec_space_induced}

\red{I think that the notation in Figures 2 and 3 are incompatible and they are further incompatible with the notation in the manuscript. Am I right?}

We provide a different perspective to think of networks as semimetric spaces where: (i) There are interior points defined by convex combinations of given nodes. (ii) Dissimilarities between these interior points are determined by the dissimilarities between the original points. To substantiate the formal definition below (Definition \ref{dfn_induced_space}) we discuss the problem of defining the interior of a network with three points. Such network is illustrated in Figure \ref{fig_inside_example} where nodes are denoted as $a$, $b$, and $c$ and dissimilarities are denoted as $d_X$. Our aim is to induce a space $(S_X, s_X)$ where the dissimilarities in the induced space are $s_X : S_X \times S_X \rightarrow \reals_+$. We require that $S_X$ preserve the distance of original points in $N_X$ such that $s_X(a, b) = r_X(a, b)$, $s_X(a, c) = r_X(a, c)$, and $s_X(b, c) = r_X(b,c)$. 

Points inside the network are represented in terms of convex combinations of the original points $a$, $b$, and $c$. Specifically, a point $m$ in the interior of the network is represented by the tuple $(m_a, m_b, m_c)$ which we interpret as indicating that $m$ contains an $m_a$ proportion of $a$, an $m_b$ proportion of $b$, and an $m_c$ proportion of $c$. Points $e$, $f$, and $g$ on Figure \ref{fig_inside_example} contain null proportions of some nodes and are interpreted as lying on the edges. Do notice that although we are thinking of $m$ as a point inside the triangle, a geometric representation does not hold. 

To specify dissimilarities $s_X$ between points on the edges and the original nodes we stipulate that node proportions be translated into dissimilarity proportions. E.g., if we consider the point $e = \alpha a + (1-\alpha)b$, we say that we must have $s_X(a, e) = \alpha r_X(a, b)$ and $s_X(b,e) = (1-\alpha) r_X(a, b)$. The dissimilarity to point $c$ is stipulated to be $s_X(e, c) = \alpha r_X(a, c) + (1-\alpha) r_X(b, c)$ because we passed the proportions that $e$ contains of $a$ and $b$ into proportions that hold for the dissimilarities $r_X(a, c)$ and $r_X(b, c)$ between $a$ and $b$ with the point of interest $c$. \green{We emphasize that these are arbitrary choices.} \red{Not sure, they have a rationale, but I am failing to explain.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centerline{\input{figures/arbitrary_points}\vspace{-4mm}
 }
\caption{Comparing arbitrary points inside the space induced from networks of three nodes. Given a pair of nodes $p$ and $m$ in the induced space, we need to find paths from $p$ to $m$ that are consisted of vectors parallel to the direction of original nodes in the networks, e.g. $a$ to $b$, $a$ to $c$, and/or $b$ to $c$. We assume the direction of original nodes in the networks have unit amount of transformation. Potential choices of paths from $p$ to $m$ include: $p$ to $m$ via $q_1$, via $q_2$, or via $q_3$. Of them, the path $p$ to $m$ via $q_1$ has the smallest amount of transformation traversed along the path. There are paths in the form which involves vectors $p$ to $q_2$, $q_2$ to $q_4$, and $q_4$ to $m$; such paths would not give the optimal solution to \eqref{eqn_constraint_arbitraryNodes}.\vspace{-4mm}
}
\label{fig_arbitrary_points}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\green{For arbitrary points $m$ and $p$ with respective tuple representation $(m_a, m_b, m_c)$ and $(p_a, p_b, p_c)$ in the space induced from the network of three nodes (Figure \ref{fig_arbitrary_points}), if we want to define their distance only by leveraging the original known relationships -- $r_X(a, b)$, $r_X(a, c)$, and/or $r_X(b, c)$, we need to find paths connecting them consisted of line segments parallel to the directions $a$ to $b$, $a$ to $c$, and/or $b$ to $c$. Three paths would satisfy the requirements: $pq_1$ followed by $q_1m$, $pq_2$ followed by $q_2m$, and $pq_3$ followed by $q_3m$. Other paths, e.g. $pq_4$ followed by $q_4q_2$ followed by $q_2m$, would be unreasonable since they would consist of back-and-force paths. Out of three reasonable paths, the one with $pq_1$ followed by $q_1m$ is desired. This is because if we consider that it takes one {\it unit of transformation} to transform any original node in the network, to another original node (for example, transform $a$ to $b$, or to transform $b$ to $c$), then the path $pq_1$ followed by $q_1m$ yields the smallest amount of total transformation. To formalize this intuition, we define $w_{ab}$ as the proportion of the path parallel to the direction $a$ to $b$ that is traversed when we connect $p$ to $m$. This implies the amount of changes from $p$ to $m$ that results from the difference from $a$ to $b$. The weight $w_{ab}$ has sign: when $w_{ab}$ is positive, it means $m$ is more similar to $b$ and $p$ is more similar to $a$; $w_{ab}$ is negative if the converse holds; $w_{ab} = 0$ if the difference between $p$ and $m$ does not result from the dissimilarity between $a$ and $b$. We can define $w_{ba}$ as the amount of change from $p$ to $m$ that results from the difference from $b$ to $a$; however it is obvious that $w_{ba} = -w_{ab}$ and therefore we only consider $w_{ab}$. Weights $w_{ac}$ and $w_{bc}$ are defined similarly. The problem then becomes trying to a path from $p$ to $m$ yielding the smallest amount of transformation, i.e. we find $w_{ab}^\star, w_{bc}^\star, w_{ac}^\star$ for the following problem
%
\begin{equation}\begin{aligned}\label{eqn_constraint_threeNodes}
    \min \quad & \left| w_{ab} \right| + \left| w_{ac} \right| + \left| w_{bc} \right| \\
    \st \quad & m_a = p_a - w_{ab} - w_{ac}, \\
    & m_b = p_b + w_{ab} - w_{bc}, \\
    & m_c = p_c + w_{ac} + w_{bc}.
\end{aligned}\end{equation}
%
The problem in \eqref{eqn_constraint_threeNodes} can always be solved since \eqref{eqn_constraint_threeNodes} is underdetermined due to the facts that $m_a + m_b + m_c = p_a + p_b + p_c = 1$. The dissimilarity between $p$ and $m$ is then the dissimilarity traversed according to the path yielding the smallest amount of transformation. In the case examined in Figure \ref{fig_arbitrary_points}, the length of the path from $p$ to $m$ is $|w_{ab}^\star| + |w_{bc}^\star|$ and their distance is
%
\begin{align}\label{eqn_threeNode_pmDistance}
    s_X(p, m) = \left|w_{ab}^\star\right| r_X(a,b) + \left|w_{bc}^\star\right| r_X(b,c).
\end{align}
%
It can be easily verified that when $p$ and/or $m$ is on the edge, this construction yields the desired property we derived before.} \blue{We need to rewrite.}

Given any network with arbitrary number of nodes, we define the induced space as a generalization to the case for nodes with three nodes we developed previously.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_induced_space}
Given a network $N_X = (X, r_X)$ with $X = \{1, 2, \dots, n\}$, the induced space $(S_X, s_X)$ is defined such that the space $S_X$ is the convex hull of $X$ with $S_X = \{m = (m_1, m_2, \dots, m_n) \mid m_i \geq 0, \sum_{i\in X} m_i = 1\}$. Given a pair of nodes $m, p \in S_X$, the path yielding the smallest amount of transformation from $p$ to $m$ is obtained through the problem
%
\begin{equation}\begin{aligned}\label{eqn_constraint_arbitraryNodes}
    \left\{ w_{ij}^\star \right\} = \argmin ~ & \sum_{i, j \in X, i < j}\left| w_{ij} \right| \\
    \st ~ & m_i = p_i - \!\! \sum_{j \in X, j > i} w_{ij} + \!\!\sum_{j \in X, j < i} w_{ji}, ~ \forall i
\end{aligned}\end{equation}
%
The distance between $p$ and $m$ is then the distance traversed proportional to the original relationships weighted by the path,
%
\begin{align}\label{eqn_arbitrary_pmDistance}
    s_X(p, m) = \sum_{i, j \in X, i< j}\left|w_{ij}^\star\right| r_X(i, j).
\end{align}\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The induced space $S_X$ is the convex hull constructed by all nodes $i \in X$. Each node in the induced space $m \in S_X$ can be represented as a tuple $(m_1, m_2, \dots, m_n)$ with $\sum_{i \in X}m_i = 1$ where $m_i$ represents the percentage of $m$ inheriting the property of node $i \in X$. To come up with distance between pairs of points $p, m \in S_X$ with the respective tuple representation $(p_1, p_2, \dots, p_n)$ and $(m_1, m_2, \dots, m_n)$, we consider each edge in the original space $X$, e.g. from $i$ to $j$, represents one unit of cost to transform $i$ into $j$. All edges are considered similarly with one unit of cost to transform the starting node into the ending node. We want to find the smallest amount of cost to transform $p$ into $m$. This is solved via \eqref{eqn_constraint_arbitraryNodes}, which is always solvable since the problem is underdetermined due to the facts that $\sum_{i \in X}m_i = \sum_{i \in X}p_i = 1$. This gives us the optimal path with weights $\{w_{ij}^\star\}$ meaning that the most cost-saving transformation from $p$ into $m$ is to undertaking $w_{ij}^\star$ unit of transformation along the direction of transforming $i$ into $j$. The distance in the induced space $s_X(p, m)$ is then the distance traversed proportional to the original relationships weighted by the path defined in \eqref{eqn_arbitrary_pmDistance}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition}\label{prop_semimetric}
The space $(S_X, s_X)$ induced from $N_X = (X, r_X)$ defined in Definition \ref{dfn_induced_space} is a semimetric space in $S_X$. Moreover, the induced space preserves relationships: when $p, m \in X$, $s_X(p, m) = r_X(p, m)$.
\end{proposition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   O   F   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{myproof} See Appendix \ref{apx_proof_2} for proofs in Section \ref{sec_space_induced}. \end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The semimetric established in Proposition \ref{prop_semimetric} guarantees that the points in the induced space with their dissimilarity $s_X(p, m)$ are well-behaved. We note that semimetric is the best property we can expect, since the triangle inequality may not be satisfied even for the dissimilarities in the original networks. Next we show that the embedding distance is preserved when interiors are considered.



==> Versions/V3_package/sec_4a_distance_equivalance_sample.tex <==
%!TEX root = journal_network_embedding.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Distances between Networks extended to their Interiors}\label{sec_interior_distance}

Since semimetrics are induced purely from the relationships in the original network, a pair of networks $N_X$ and $N_Y$ can be compared by considering their induced space, as we state next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_induced_space_distance}
Given two networks $N_X = (X, r_X)$ and $N_Y = (Y, r_Y)$ with their respective induced space $(S_X, s_X)$ and $(S_Y, s_Y)$, for a map $\phi: S_X \rightarrow S_Y$ from the induced space $S_X$ to the induced space $S_Y$ such that $\phi(x) \in Y$ for any $x\in X$, define the network difference with respect to $\phi$ as 
%
\begin{align}\label{eqn_dfn_induced_space_distance_prelim}
    \Delta_{S_X, S_Y} (\phi)
         :=  \max_{x, x' \in S_X} 
            \Big| s_X(x, x') - s_Y (\phi(x),\phi(x')) \Big|.
\end{align}
%
The partial embedding distance from $N_X$ to $N_Y$ measured with respect to the induced spaces is then defined as
%
\begin{align}\label{eqn_dfn_induced_space_distance}
   d_\PES(N_X, N_Y) := \min_{\phi: S_X \rightarrow S_Y \mid \phi(x) \in Y, \forall x\in X } 
    \Big\{ \Delta_{S_X, S_Y} (\phi) \Big\}.
\end{align} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The partial embedding distance $d_\PES(N_X, N_Y)$ with respect to the induced space in \eqref{eqn_dfn_induced_space_distance} is defined similarly as the partial embedding distance $d_\PE(N_X, N_Y)$ in \eqref{eqn_dfn_partial_embedding} however considers the mapping between all elements in the induced spaces. %By the second part of Proposition \ref{prop_semimetric}, $s_X$ incorporates all information in $r_X$ and similarly for $s_Y$. Therefore, comparing the original networks via the induced spaces is reasonable. Simultaneously, since the induced space is richer, the problem where different networks result in identical multi-dimensional scaling results illustrated in Figure \ref{fig_mds_original} would be alleviated. 
Observe that we further require that the embedding satisfy $\phi(x) \in Y$ for any $x\in X$. This ensures the original nodes of network $X$ are mapped to original nodes of network $Y$. The restriction is incorporated because it makes the embedding distance $d_\PES(N_X, N_Y)$ with respect to the induced spaces identical to the original embedding distance $d_\PE(N_X, N_Y)$ as we state next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[t]
\centerline{\input{figures/regular_sample_pair}\vspace{-3mm} 
}
\caption{An example of regular sample pair $(Q_X, \hhatr_X)$ and $(Q_Y, \hhatr_Y)$, where $Q_X = \{a, b, c, x_1, x_2, x_3, x_4, x_5, x_6, p\}$ collects original points and induced points that are combination of one-third of original nodes, and $Q_Y = \{u, v, y_1, y_2\}$. Here we illustrate a specific mapping $\hhatphi$ with $\hhatphi(a) = \hhatphi(b) = u$ and $\hhatphi(c) = v$; it is apparent that $\phi(x) \in Q_Y$ for any $x \in Q_X$. Note that $\tdQ_X = Q_X / \{q\}$ also form a regular sample pair with $Q_Y$.\vspace{-3mm}
}
\label{fig_regular_sample_pair}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem}\label{thm_induced_space_distance_same}
The function $d_\PES: \ccalN \times \ccalN \rightarrow \reals_+$ defined in \eqref{eqn_dfn_induced_space_distance} is an embedding metric in the space $\ccalN$ and  yields the same distance as the function $d_\PE$ defined in \eqref{eqn_dfn_partial_embedding}, 
%
\begin{align}\label{eqn_thm_induced_space_distance_same}
    d_\PES(N_X, N_Y) = d_\PE(N_X, N_Y),
    \quad \text {for all\ } N_X, N_Y.
\end{align} \end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[t]
\centerline{\input{figures/embedding_sample_3.tex}\vspace{-1mm} 
}
\begin{minipage}[h]{0.032\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_1.eps}
\end{minipage}
\begin{minipage}[h]{0.054\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_2.eps}
\end{minipage}
\begin{minipage}[h]{0.054\textwidth}
~
\end{minipage}
\begin{minipage}[h]{0.275\textwidth}
    	\centering
    	\includegraphics[trim=0.01cm 0.01cm 0.01cm 0.01cm, clip=true, width=1 \textwidth]
	{figures/mds_3.eps}
\end{minipage}
\caption{The caveat illustrated in Figure \ref{fig_mds_original} where different networks results in identical multi-dimensional scaling results could be solved by considering the induced sample space where we utilize the same predetermined sampling strategy -- taking midpoints for all edges -- in the network. Multi-dimensional scaling by adding interiors would distinguish different networks. The dissimilarities between nodes $a$ and $f$ are not illustrated in the respective induced network due to space limit.\vspace{-3mm}
}
\label{fig_mds_midpoints}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The statement in Theorem \ref{thm_induced_space_distance_same} justifies comparing networks via their respective induced space. Similar as in Definition \ref{dfn_embedding}, defining $\max\{d_\PES(N_X, N_Y), d_\PES(N_Y, N_X)\}$ would yield a metric in the space $\ccalN \mod \cong$ and this maximum is the same as $d_\EE$ defined in \eqref{eqn_dfn_embedding}. Since the induced spaces incorporate more information of the original networks while at the same time $d_\PES(N_X, N_Y) = d_\PE(N_X, N_Y)$, an approximation to $d_\PES(N_X, N_Y)$ via the induced space would be a better approximation to $d_\PE(N_X, N_Y)$. It may appear that the evaluation of the induced space is costly. However, we demonstrate in the next subsection that the partial embedding distances have a nice property that if we sample a number of points in the induced spaces respectively according to the same rule, the distance between the sampled induced space is the same as the original distance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Sampling of Interiors}\label{sec_partial_embedding_induced}

In this section, we consider a practical scenario where we only take several samples in the induced space. We show that comparing the combination of nodes in the respective original networks and sampled nodes in the induced space would yield the same result as comparing the original networks. Given a network $N_X = (X, r_X)$, our aim is to define a sampled induced space $(Q_X, \hhatr_X)$ where $Q_X \supset X$ includes more nodes compared to $X$. An example is in Figure \ref{fig_mds_midpoints}, where the original node space is given by $\{a, b, c\}$, and one version of sampled induced node space is $Q_X = \{a, b, c, e, f, g\}$, the union of the original nodes and the nodes in the midpoints of the edges in the original networks. The distance in the sampled induced space $\hhatr_X: Q_X \times Q_X \rightarrow \reals_+$ should preserve the distance of original points in $X$. A natural choice for $\hhatr_X$ is the restriction of the distance $s_X$ defined for the induced space $S_X$: i.e. given any pair of points $x, x' \in Q_X$, let $\hhatr_X(x, x') := s_X(x, x')$. Our key observation for such construction is that if the nodes in the induced spaces of a pair of networks are sampled according to the same strategy, then the distance between the sampled induced space is identical to the original distance. We start by formally describing what do we mean by a pair of networks sampled according to the same rule as next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_sample_same_rule}
Given a pair of networks $N_X = (X, r_X)$ and $N_Y = (Y, r_Y)$, their respective sampled induced space $(Q_X, \hhatr_X)$ and $(Q_Y, \hhatr_Y)$ form a regular sample pair, if for any mapping $\hhatphi: X \rightarrow Y$ in the original node set, we have $\phi(x) \in Q_Y$ for any $x \in Q_X$ where $\phi: S_X \rightarrow S_Y$ is the map induced from $\hhatphi$ such that $\phi: x \mapsto \phi(x)$ whose the $i$-th element in the tuple representation $[\phi(x)]_i$ is given by
%
\begin{align}\label{eqn_dfn_sample_same_rule_phi_mapping}
    [\phi(x)]_i = \sum_{j \in X} \bee{\hhatphi(j) = i} x_j,
\end{align}
%
and for any mapping $\hhatpsi: Y \rightarrow X$ in the original node set, we have $\psi(y) \in Q_X$ for any $x \in Q_X$ where $\psi: S_Y \rightarrow S_X$ is the map induced from $\hhatpsi$ such that the $i$-th element in the tuple representation of $\psi(y)$ is 
%
\begin{align}\label{eqn_dfn_sample_same_rule_psi_mapping}
    [\psi(y)]_i = \sum_{j \in Y} \bee{\hhatpsi(j) = i} y_j.
\end{align}
%
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\noindent In the definition, $\beeInline{\hhatphi(j) = i}$ is the indicator function such that it equals one if $\hhatphi$ maps $j\in X $ to $i\in Y$ and $\beeInline{\hhatphi(j) = i} = 0$ otherwise. It is easy to see that $\phi$ in \eqref{eqn_dfn_sample_same_rule_phi_mapping} is well-defined. Firstly, $[\phi(x)]_i \geq 0$ for any $i \in Y$, and
%
\begin{align}\label{eqn_dfn_sample_same_rule_phi_mapping_proof}
    \sum_{i \in Y}[\phi(x)]_i = \sum_{i \in Y}\sum_{j \in X} \bee{\hhatphi(j) = i} x_j 
        = \sum_{j \in X} x_j = 1,
\end{align}
%
ensuring $\phi(x)$ is in the induced convex hull space $S_Y$. Secondly, for any $j \in X$ in the original nodespace, its mapping $\phi(j)$ would have the tuple representation with $[\phi(j)]_i = \beeInline{\hhatphi(j) = i}$, a node in the original node space of $Y$. Consequently, for any $j \in X$, we have that $\phi(j) \in Y$. Combining these two observations imply that $\phi: S_X \rightarrow S_Y$ is well-defined. By symmetry, $\psi$ induced from $\hhatpsi$ is also well-defined from $S_Y$ to $S_X$. Definition \ref{dfn_sample_same_rule} states that for any point $x$ in $Q_X$, no matter how we relate points in $Q_X$ to points in $Q_Y$, the mapped node $\phi(x)$ should be in the induced sample space $Q_Y$. An example of regular sample pair is illustrated in Figure \ref{fig_regular_sample_pair}, where $Q_X = \{a, b, c, x_1, x_2, x_3, x_4, x_5, x_6, p\}$ is the collection of original node space and points that are combination of one-third of original nodes and $Q_Y = \{u, v, y_1, y_2\}$. Figure \ref{fig_regular_sample_pair} exemplifies the scenario for a specific mapping $\hhatphi$ with $\hhatphi(a) = \hhatphi(b) = u$ and $\hhatphi(c) = v$; it is apparent that $\phi(x) \in Q_Y$ for any $x \in Q_X$. We note that $\tdQ_X = Q_X / \{q\}$ also form a regular sample pair with $Q_Y$. A pair of networks $N_X$ and $N_Y$ can be compared by evaluating their difference in their respective sampled induced space as next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}\label{dfn_sampled_space_distance}
Given two networks $N_X = (X, r_X)$ and $N_Y = (Y, r_Y)$ with their respective sampled induced space $(Q_X, \hhatr_X)$ and $(Q_Y, \hhatr_Y)$, for a map $\phi: Q_X \rightarrow Q_Y$ such that $\phi(x) \in Y$ for any $x\in X$, define the difference with respect to $\phi$ as 
%
\begin{align}\label{eqn_dfn_sampled_space_distance_prelim}
    \Delta_{Q_X, Q_Y} (\phi)
         :=  \max_{x, x' \in Q_X} 
            \Big| \hhatr_X(x, x') - \hhatr_Y (\phi(x),\phi(x')) \Big|.
\end{align}
%
The partial embedding distance from $N_X$ to $N_Y$ measured with respect to the sampled induced spaces is then defined as
%
\begin{align}\label{eqn_dfn_sampled_space_distance}
   d_\PEQ(N_X, N_Y) := \min_{\phi: Q_X \rightarrow Q_Y \mid \phi(x) \in Y, \forall x\in X } 
    \Big\{ \Delta_{Q_X, Q_Y} (\phi) \Big\}.
\end{align} \end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Our key result is that $d_\PEQ(N_X, N_Y)$ is the same as the partial embedding distance $d_\PE(N_X, N_Y)$ defined in \eqref{eqn_dfn_partial_embedding} when the sampled space form a regular sample pair.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[t]
\begin{minipage}[h]{0.40\linewidth}
    	\centering
    	\input{figures/simple_points.tex}
\end{minipage}
\begin{minipage}[h]{0.025\linewidth}
        ~
\end{minipage}
\begin{minipage}[h]{0.24\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/distance_middle.eps}
	{\scriptsize (b) with interiors}
\end{minipage}
\begin{minipage}[h]{0.025\linewidth}
        ~
\end{minipage}
\begin{minipage}[h]{0.24\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/distance_noMiddle.eps}
	{\scriptsize (c) without interiors}
\end{minipage}
\caption{Example of the usefulness of considering the interior of networks. We consider 10 networks in the form (a) where $\gamma = 1, 2, \dots, 10$. Approximations of network embedding distances are evaluated. (b) and (c) illustrate the heat-maps of the distance approximations where the indices in both horizontal and vertical directions denote $\gamma$ in the networks. When interiors are considered by adding midpoints of edges, e.g. nodes $e$, $f$, and $g$ in (a), network distance approximations (b) yield more desired results, especially for $\gamma \leq 5$ where the relationships in the original networks fail to satisfy triangle inequality.}
\label{fig_application_0}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[t]
\begin{minipage}[h]{0.246\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/mds_mid_25_nodes.eps}
	{\scriptsize (a) with interiors, $25$ nodes}
\end{minipage}
\begin{minipage}[h]{0.246\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/mds_noM_25_nodes.eps}
	{\scriptsize (b) without interiors, $25$ nodes}
\end{minipage}
\begin{minipage}[h]{0.246\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/mds_mid_20_30_nodes.eps}
	{\scriptsize (c) with interiors, $20$ to $25$ nodes}
\end{minipage}
\begin{minipage}[h]{0.246\linewidth}
    	\centering
    	\includegraphics[trim=1.5cm 0.9cm 1.5cm 0.7cm, clip=true, width=1 \textwidth]
	{figures/mds_noM_20_30_nodes.eps}
	{\scriptsize (d) without interiors, $20$ to $25$ nodes}
\end{minipage}
\caption{Two dimensional Euclidean embeddings of the networks constructed from three different models with different number of nodes with respect to the approximation to the network embedding distance. In the embeddings, red circles denote networks constructed from the Erd\H os-R\' enyi model, blue diamonds represent networks constructed from the unit circle model, and black squares the networks from the correlation model.\vspace{-4mm}
}
\label{fig_application}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   T   H   E   O   R   E   M   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem}\label{thm_sampled_induced_space}
When the sampled spaces $Q_X$ and $Q_Y$ form a regular sample pair, the function $d_\PEQ: \ccalN \times \ccalN \rightarrow \reals_+$ defined in \eqref{eqn_dfn_sampled_space_distance_prelim} is an embedding metric in the space $\ccalN$. Moreover, it yields the same distance as the function $d_\PE$ defined in \eqref{eqn_dfn_partial_embedding}, i.e.
%
\begin{align}\label{eqn}
    d_\PEQ(N_X, N_Y) = d_\PE(N_X, N_Y),
\end{align}
%
for any networks $N_X$ and $N_Y$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N      M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The statement in Theorem \ref{thm_sampled_induced_space} gives proper reasoning for differentiating networks via their sampled induced space. Similar as previous treatments, we could define $\max\{d_\PEQ(N_X, N_Y), d_\PEQ(N_Y, N_X)\}$ as a metric in the space $\ccalN \mod \cong$. Since the sampled induced spaces incorporate more information of the original networks, an approximation to $d_\PEQ(N_X, N_Y)$ via the sampled induced space would be a better approximation to $d_\PE(N_X, N_Y)$. Moreover, since we can construct the sampled induced space following some predetermined strategy -- taking midpoints for all edges in the networks, comparing networks via their sampled induced space is plausible in terms of complexity. Figure \ref{fig_mds_midpoints} illustrate the same network considered in Figure \ref{fig_mds_original} where the multi-dimensional scaling based on the sampled induced points would succeed in distinguishing networks that are different. We illustrate the practical usefulness of such methods in the next section.


==> Versions/V3_package/sec_5_application.tex <==
%!TEX root = journal_network_embedding.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Application}\label{sec_application}

We first illustrate the usefulness of considering interiors of networks. We consider 10 networks in the form Figure \ref{fig_application_0} (a) where $\gamma = 1, 2, \dots, 10$. Approximations of network embedding distances are evaluated. Figure \ref{fig_application_0} (b) and (c) illustrate the heat-maps of the distance approximations where the indices in both horizontal and vertical directions denote the value of $\gamma$ in the networks. When interiors are considered by adding midpoints of edges, e.g. nodes $e$, $f$, and $g$ in Figure \ref{fig_application_0} (a), network distance approximations illustrated in Figure \ref{fig_application_0} (b) yield more desired results, as networks with similar $\gamma$ are close to each other with respect to their network distance approximations. This is more apparent for networks with $\gamma \leq 5$, where the relationships in the original networks fail to satisfy triangle inequality. A detailed analysis indicates that adding interior points in the networks (i) preserve the desired property of embedding distance when interiors are not considered (the distance approximations in Figure \ref{fig_application_0} (b) and (c) are very similar for $\gamma > 5$ where triangle inequalities are satisfied) and (ii) fix the undesired issue when the relationships in the original networks fail to satisfy triangle inequality.

We next consider the comparison and classification of three types of synthetic weighted networks. Edge weights in all three types of networks encode proximities. The first type of networks are with weighted Erd\H os-R\' enyi model \cite{erd6s1960}, where the edge weight between any pair of nodes is a random number uniformly selected from the unit interval $[0, 1]$. In the second type of networks, the coordinates of the vertices are generated uniformly and randomly in the unit circle, and the edge weights are evaluated with the Gaussian radial basis function $\exp(-d(i,j)^2 / 2\sigma^2)$ where $d(i,j)$ is the distance between vertices $i$ and $j$ in the unit circle and $\sigma$ is a kernel width parameter. In all simulations, we set $\sigma$ to $0.5$. The edge weight measures the proximity between the pair of vertices and takes value in the unit interval. In the third type of networks, we consider that each vertex $i$ represents an underlying feature $\bbu_i \in \reals^d$ of dimension $d$, and examine the Pearson's linear correlation coefficient $\rho_{ij}$ between the corresponding features $\bbu_i$ and $\bbu_j$ for a given pair of nodes $i$ and $j$. The weight for the edge connecting the pair is then set as $\rho_{ij} / 2 + 0.5$, a proximity measure in the unit interval. The feature space dimension $d$ is set as $5$ in all simulations. We want to see if network comparison tools proposed succeed in distinguishing networks generated from different processes.

We start with networks of equal size $|X| = 25$ and construct $20$ random networks for each aforementioned type. We then use the multi-dimensional scaling methods introduced in \cite{bronstein2006, bronstein2006a} to approximate the embedding network distance $d_\EE$ defined in Definition \ref{dfn_embedding}. To evaluate the effectiveness of considering interiors of networks described in Section \ref{sec_space_induced}, we add midpoints for all edges in a given network; it is apparent that any pair of networks with interiors defined in this way would form a regular sample pair. Approximations of the embedding network distance $d_\EE$ between these networks with midpoints added are then evaluated. Figure \ref{fig_application} (a) and (b) plot the two dimensional Euclidean embeddings \cite{CoxCox08} of the network metric approximations with and without interiors respectively. All embeddings in the paper are constructed with respect to minimizing the sum of squares of the inter-point distances; other common choices to minimize the sum of four power of the inter-point distances yields similar results. Networks constructed with different models form clear separate clusters (1 out of 60 errors with 1.67\%) with respect to approximation of network distances between networks with interior points added, where networks with Erd\H os-R\' enyi model are denoted by red circles, networks with unit circle model are described by blue diamonds, and correlation model represented as black squares. The clustering structure is not that clear (4 out of 20 errors with 6.67\%) in terms of with respect to approximation of network distances between networks without interior points, but networks constructed from different models are in general much more different compared to networks from the same model. 

Next we consider networks with number of nodes ranging between $20$ and $25$. Two networks are randomly generated for each network type and each number of nodes, resulting in $60$ networks in total. Interiors are examined similarly as before by adding midpoints for all edges in a given network. Figure \ref{fig_application} (c) and (d) illustrate the two dimensional Euclidean embeddings of the network metric approximations with and without interiors respectively. Despite the fact that networks with same model have different number of nodes, dissimilarities between network distance approximations are smaller when their underlying networks are from the same process. Similar as in the case with same number of nodes, considering interiors result in a more distinctive clustering pattern. An unsupervised classification with two linear boundaries would yield 1 out of 60 errors ($1.67\%$) for networks with interiors added and 3 errors ($5\%$) without interiors.

These results illustrate that (i) comparing networks by using embedding distance succeeds in identifying networks with different properties, and (ii) adding interiors to networks to form regular sample pair as in Section \ref{sec_space_induced} would yield better approximations to the actual network distances. Admittedly, other methods to compare networks may also succeed in distinguishing networks, after some proper treatment towards the issue of different sizes. Nonetheless, interior and embedding method would be more universal, not only for the reason that it establishes an approximation to the actual network metrics, but also since it provides a systematic way to analyze if one network can be well matched to a subset of another network.








==> Versions/V3_package/sec_6_conclusion.tex <==
%!TEX root = journal_network_embedding.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Conclusion}\label{sec_conclusion}

We present a different perspective to consider networks by defining a semimetric space induced from all the relationships in a given network. We demonstrate that comparing the respective induced space between a pair of networks outputs the identical distance as evaluating the discrepancy between the original network by embedding one network into another network, which we prove to be a valid metric in the space of all networks. Therefore, better approximations to the network metric distances can be constructed by examining the respective induced space. We illustrate that such methods succeed in classifying weighted pairwise networks constructed from different processes.
